Interval Enclosures of Upper Bounds of Roundoff Errors using Semidefinite Programming

A longstanding problem related to floating-point implementation of numerical programs is to provide efficient yet precise analysis of output errors. We present a framework to compute lower bounds on largest absolute roundoff errors, for a particular rounding model. This method applies to numerical programs implementing polynomial functions with box constrained input variables. Our study is based on three different hierarchies, relying respectively on generalized eigenvalue problems, elementary computations and semidefinite programming (SDP) relaxations. This is complementary of over-approximation frameworks, consisting of obtaining upper bounds on the largest absolute roundoff error. Combining the results of both frameworks allows to get enclosures for upper bounds on roundoff errors. The under-approximation framework provided by the third hierarchy is based on a new sequence of convergent robust SDP approximations for certain classes of polynomial optimization problems. Each problem in this hierarchy can be solved exactly via SDP. By using this hierarchy, one can provide a monotone non-decreasing sequence of lower bounds converging to the absolute roundoff error of a program implementing a polynomial function, applying for a particular rounding model. We investigate the efficiency and precision of our method on non-trivial polynomial programs coming from space control, optimization and computational biology.

==> defManOcaml.tex <==
%=======================================================================
% Définit le style ssr Gallina pour les listings (Assia Mahboubi 2007)

\lstdefinelanguage{Ocaml} {

% Anything betweeen $ becomes LaTeX math mode
mathescape=true,						
% Comments may or not include Latex commands
texcl=false,


% Vernacular commands
morekeywords=[1]{
Section, Module, End, Require, Import, Export, Defensive, Function,
Variable, Variables, Parameter, Parameters, Axiom, Hypothesis, Hypotheses,
Notation, Local, Tactic, Reserved, Scope, Open, Close, Bind, Delimit,
Definition, Let, Ltac, Fixpoint, CoFixpoint, Morphism, Relation,
Implicit, Arguments, Set, Unset, Contextual, Strict, Prenex, Implicits,
Inductive, CoInductive, Record, Structure, Canonical, Coercion,
Theorem, Lemma, Corollary, Proposition, Fact, Remark, Example,
Proof, Goal, Save, Qed, Defined, Hint, Resolve, Rewrite, View,
Search, Show, Print, Printing, All, Graph, Projections, inside,
outside, Locate, Maximal, assume, procedure, 
Persistent, Digraph, ConcreteBidirectional, G 

},

% Gallina
morekeywords=[2]{match, forall, exists, exists2, fun, fix, cofix, struct,
       as, return, if, is, then, else, begin, end, 
      for,  nosimpl, at,
      
       Noedges, Gp , Fe
      
      },

% Sorts
morekeywords=[3]{Type, Prop},

% Various tactics, some are std Coq subsumed by ssr, for the manual purpose
morekeywords=[4]{ 
         type, let, pose, set, move, case, elim, apply, clear, exception, when, with, of, raise, module,
            hnf, intro, intros, generalize, rename, pattern, after, rec,
	    destruct, induction, using, refine, inversion, injection,
         rewrite, congr, unlock, compute, ring, micromega field,
            replace, fold, unfold, change, cutrewrite, simpl,
         have, suff, wlog, suffices, without, loss, nat_norm,
            assert, cut, trivial, revert, bool_congr, nat_congr,
	 symmetry, transitivity, auto, split, left, right, autorewrite},        

% Terminators
morekeywords=[5]{
         by, done, exact, reflexivity, tauto, romega, omega,
         assumption, solve, contradiction, discriminate},


% Control
morekeywords=[6]{do, last, first, try, idtac, repeat},
keywordsprefix=F
% Various symbols
% For the ssr manual we turn off the prettyprint of formulas
 literate=	
	{->}{{$\rightarrow\,$}}2		
 	{->}{{\tt ->}}3
	{<-}{{$\leftarrow\,$}}2	
 	{<-}{{\tt <-}}2			
 	{>->}{{$\mapsto$}}3		
 	{<=}{{$\leq$}}1			
 	{>=}{{$\geq$}}1		
 	{<>}{{$\neq$}}1
 	{/\\}{{$\wedge$}}2	
 	{\\/}{{$\vee$}}2 		
 	{<->}{{$\leftrightarrow\;$}}3
 	{<=>}{{$\Leftrightarrow\;$}}3
 	{:nat}{{$~\in\mathbb{N}$}}3	
	{fforall\ }{{$\forall_f\,$}}1		
	{forall\ }{{$\forall\,$}}1		
	{exists\ }{{$\exists\,$}}1
 	{negb}{{$\neg$}}1
 	{spp}{{:*:\,}}1
 	{~}{{$\sim$}}1
 	{\\in}{{$\in\;$}}1
 	{/\\}{$\land\,$}1
 	{:*:}{{$*$}}2
	{=>}{{$\,\Rightarrow\ $}}1
 	{=>}{{\tt =>}}2
 	{:=}{{{\tt:=}\,\,}}2
 	{==}{{$\equiv$}\,}2
 	{!=}{{$\neq$}\,}2
 	{^-1}{{$^{-1}$}}1
 	{elt'}{elt'}1
       {=}{{\tt=}\,\,}2
       {+}{{\tt+}\,\,}2,
literate=
	{isn't }{{{\ttfamily\color{dkgreen} isn't }}}1,

% Comments delimiters, we do turn this off for the manual
comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% String delimiters
morestring=[b]",
morestring=[d]',

% Size of tabulations
tabsize=3,							

% Enables ASCII chars 128 to 255
extendedchars=true,  		 		

% Case sensitivity
sensitive=true, 

% Automatic breaking of long lines
breaklines=true,

% Default style fors listings
basicstyle=\ttfamily,

% Position of captions is bottom
captionpos=b,							

% Full flexible columns 
columns=fixed,%fullflexible,

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
%keywordstyle=[1]{\ttfamily\color{black}},
keywordstyle=\bfseries,
% Style for gallina keywords
%keywordstyle=[2]{\ttfamily\color{black}},

% Style for sorts keywords
%keywordstyle=[3]{\ttfamily\color{lightblue}},

% Style for tactics keywords
%keywordstyle=[4]{\ttfamily\color{dkblue}},

% Style for terminators keywords
%keywordstyle=[5]{\ttfamily\color{red}},


%Style for iterators
%keywordstyle=[6]{\ttfamily\color{dkpink}},
%keywordstyle=[7]{\ttfamily\color{dkgreen}},
% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle=\rmfamily,

}

%=======================================================================
% Définit le style ssr Gallina pour les listings (Assia Mahboubi 2007)

\lstdefinelanguage{NLCertify} {

% Anything betweeen $ becomes LaTeX math mode
mathescape=true,						
% Comments may or not include Latex commands
texcl=false,


% Vernacular commands
morekeywords=[1]{
Section, Module, End, Require, Import, Export, Defensive, Function,
Variable, Variables, Parameter, Parameters, Axiom, Hypothesis, Hypotheses,
Notation, Local, Tactic, Reserved, Scope, Open, Close, Bind, Delimit,
Definition, Let, Ltac, Fixpoint, CoFixpoint, Morphism, Relation,
Implicit, Arguments, Set, Unset, Contextual, Strict, Prenex, Implicits,
Inductive, CoInductive, Record, Structure, Canonical, Coercion,
Theorem, Lemma, Corollary, Proposition, Fact, Remark, Example,
Proof, Goal, Save, Qed, Defined, Hint, Resolve, Rewrite, View,
Search, Show, Print, Printing, All, Graph, Projections, inside,
outside, Locate, Maximal,
Persistent, Digraph, ConcreteBidirectional, G

},

% Gallina
morekeywords=[2]{match, forall, exists, exists2, fun, fix, cofix, struct,
       as, return, if, is, then, else, begin, end, 
      for,  nosimpl, at,
      
       Noedges, Gp , Fe
      
      },

% Sorts
morekeywords=[3]{Type, Prop},

% Various tactics, some are std Coq subsumed by ssr, for the manual purpose
morekeywords=[4]{ 
         type, let, pose, set, move, case, elim, apply, clear, exception, when, with, of, raise, module,
            hnf, intro, intros, generalize, rename, pattern, after, rec,
	    destruct, induction, using, refine, inversion, injection,
         rewrite, congr, unlock, compute, ring, micromega field,
            replace, fold, unfold, change, cutrewrite, simpl,
         have, suff, wlog, suffices, without, loss, nat_norm,
            assert, cut, trivial, revert, bool_congr, nat_congr,
	 symmetry, transitivity, auto, split, left, right, autorewrite},        

% Terminators
morekeywords=[5]{
         by, done, exact, reflexivity, tauto, romega, omega,
         assumption, solve, contradiction, discriminate},


% Control
morekeywords=[6]{do, last, first, try, idtac, repeat},
keywordsprefix=F
% Various symbols
% For the ssr manual we turn off the prettyprint of formulas
% literate=	
%	{->}{{$\rightarrow\,$}}2		
% 	{->}{{\tt ->}}3
%	{<-}{{$\leftarrow\,$}}2	
% 	{<-}{{\tt <-}}2			
% 	{>->}{{$\mapsto$}}3		
% 	{<=}{{$\leq$}}1			
% 	{>=}{{$\geq$}}1		
% 	{<>}{{$\neq$}}1
% 	{/\\}{{$\wedge$}}2	
% 	{\\/}{{$\vee$}}2 		
% 	{<->}{{$\leftrightarrow\;$}}3
% 	{<=>}{{$\Leftrightarrow\;$}}3
% 	{:nat}{{$~\in\mathbb{N}$}}3	
%	{fforall\ }{{$\forall_f\,$}}1		
%	{forall\ }{{$\forall\,$}}1		
%	{exists\ }{{$\exists\,$}}1
% 	{negb}{{$\neg$}}1
% 	{spp}{{:*:\,}}1
% 	{~}{{$\sim$}}1
% 	{\\in}{{$\in\;$}}1
% 	{/\\}{$\land\,$}1
% 	{:*:}{{$*$}}2
%	{=>}{{$\,\Rightarrow\ $}}1
% 	{=>}{{\tt =>}}2
% 	{:=}{{{\tt:=}\,\,}}2
% 	{==}{{$\equiv$}\,}2
% 	{!=}{{$\neq$}\,}2
% 	{^-1}{{$^{-1}$}}1
% 	{elt'}{elt'}1
%       {=}{{\tt=}\,\,}2
%       {+}{{\tt+}\,\,}2,
literate=
	{isn't }{{{\ttfamily\color{dkgreen} isn't }}}1,

% Comments delimiters, we do turn this off for the manual
comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% String delimiters
morestring=[b]",
morestring=[d]',

% Size of tabulations
tabsize=3,							

% Enables ASCII chars 128 to 255
extendedchars=true,  		 		

% Case sensitivity
sensitive=true, 

% Automatic breaking of long lines
breaklines=true,

% Default style fors listings
basicstyle=\ttfamily,

% Position of captions is bottom
captionpos=b,							

% Full flexible columns 
columns=fixed,%fullflexible,

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{black}},

% Style for gallina keywords
keywordstyle=[2]{\ttfamily\color{black}},

% Style for sorts keywords
keywordstyle=[3]{\ttfamily\color{black}},

% Style for tactics keywords
keywordstyle=[4]{\ttfamily\color{black}},

% Style for terminators keywords
keywordstyle=[5]{\ttfamily\color{black}},


%Style for iterators
keywordstyle=[6]{\ttfamily\color{black}},
keywordstyle=[7]{\ttfamily\color{black}},
% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle=\rmfamily,

}
